Deep multi-scale architectures for monocular depth estimation

This paper aims at understanding the role of multi-scale information in the estimation of depth from monocular images. More precisely, the paper investigates four different deep CNN architectures, designed to explicitly make use of multi-scale features along the network, and compare them to a state-of-the-art single-scale approach. The paper also shows that involving multi-scale features in depth estimation not only improves the performance in terms of accuracy, but also gives qualitatively better depth maps. Experiments are done on the widely used NYU Depth dataset, on which the proposed method achieves state-of-the-art performance.

==> metrics.tex <==
\section{Toward novel metrics for the evaluation of depth estimation}
\label{sec:metrics}

All the papers presented in the literature --  we also stick to this methodology in our experiments to make performance comparable --  evaluate the quality of the estimation through the following criteria adapted to depth estimation task:

\begin{itemize}
\item Mean relative error (rel): $\frac{1}{N}\sum_{i=1}^{N} \left |  \hat{y_{i}} - y_{i} \right | / y_{i}$
\item Mean $log_{10}$ error (log): $\frac{1}{N}\sum_{i=1}^{N}\left | log_{10} \ \hat{y_{i}}-log_{10} \ y_{i} \right |$
\item RMSE (rms): $\sqrt{\frac{1}{N}\sum_{i=1}^{N} \left ( \hat{y_{i}} - y_{i} \right )^{2}}$
\item Threshold: \% of $y_i$ s.t. $max \left ( \frac{\hat{y_{i}}}{y_{i}}, \frac{y_{i}}{\hat{y_{i}}} \right ) = \delta < thr$
\end{itemize}
Where $\hat{y_i}$ is the predicted depth at pixels $i$ and $y_i$ is their ground-truth value, with a total number of $N$ pixels.

We experimentally observed that these metrics do not reflect well the quality of the estimation. As illustrated in Figure \ref{fig:compare}, although the RMSE of the approaches are close to each other, we notice that their estimation seems very dissimilar, particularly in terms of sharpness of the depth map. At the same time, we argue that a good depth estimation should have desirable 3D properties, such as being robust to  viewpoint changes. From these two observations, we propose two new metrics that aim to capture 3D consistency and gradients sharpness of the depth map.

\subsubsection*{A novel metric based on viewpoint changes on textures}

\begin{figure}
\centering
\includegraphics[scale=0.4]{img/VCS.png}
\caption{An RGB image, its depth map and a VCS applied to the RGB image.}
\label{vcs}
\end{figure}

For each RGB test image, we use the ground-truth depth map to recover the 3D points cloud of the scene. Then, we simulate a 3D displacement of the camera before reprojecting back onto the image plane. Thus, we perform what we call a Viewpoint Change Simulation (VCS) on the RGB image, please look at Figure \ref{vcs} for an illustration. This VCS using the ground-truth depth map is now considered as our new ground truth $VCS_{GT}$. 

As a 3D consistent metric, we propose to compute a simple Mean Squared Error between the VCS obtained using an inferred depth map $VCS_{I}$ and $VCS_{GT}$.
\[ 3D-Consistent MSE = \frac{1}{N}\sum_{i=1}^{N}({VCS_{I}}_{(i)}-{VCS_{GT}}_{(i)})^{2} \]

The reprojection back onto the image plane is done using a mere nearest-neighbor algorithm. This has the effect of giving a sparse 2D image, where there are missing values on pixels that newly appeared in this new viewpoint as we can see in Figure \ref{vcs}. Here, to limit the number of occluded regions, we choose to only consider translations along x and y axis. Thus, we only have filled-in pixels when the considered point already existed in the original view. If several original pixels fall on the same destination pixel on the reconstructed image, we choose to only keep the one with the lowest depth (the closest to the camera). Therefore, the normalisation constant $N$ used in the $3D-Consistent MSE$ is the number of valid pixels.

\subsubsection*{A novel metric based on viewpoint changes on contours}

\begin{figure}
\centering
\includegraphics[scale=0.4]{img/contours.png}
\caption{An RGB image contours, a VCS applied to these contours and a map representing the Euclidean distance to the closest VCS contours.}
\label{contours}
\end{figure}

To keep the desirable property of 3D consistency, we apply the same VCS principle but only to the original RGB contours. Thereby, we want to measure the alignment between imperfect projections of RGB contours using an inferred depth map and the ones obtained using the ground truth one.

First, we compute the edges of the original RGB image using a Canny filter and binarize them. Then we apply a VCS on this binarized edge image w.r.t. the depth map. We obtain the localization of edges in the new viewpoint, as depicted in left and middle images of Figure \ref{contours}. We denote $E_{GT}$ the projected edges using a VCS computed on the ground-truth depth map and $E_{I}$ the one computed with an inferred depth map.

We calculate the distance transform of $E_{GT}$. This gives us a map where each pixel is a scalar representing the Euclidean distance from it to the closest edge pixel, as we can see in the right image of Figure \ref{contours}.
We then mask this distance map using $E_I$. What remains is an image where non-zero elements are only on the edges of $E_{I}$ and these elements are the distances to the closest $E_{GT}$ edges.

From there, the proposed metric is an average sum over the contours pixels and the images. This gives us a score representing the average distance in pixels from the edges of $E_{I}$ and the ground truth edges of $E_{GT}$.


==> old-related_work.tex <==
\section*{Related Work}
%\label{sec:related}

%\subsection*{Depth Estimation}

In the past few years, a number of deep learning methods have emerged to solve the problem of monocular depth estimation. We can roughly categorize these methods into two principal families: global methods that infer a depth map from the whole global input information, and possibly make a refinement on the obtained estimation, and local methods that work locally on image patches and possibly make a global regularization to ensure spatial consistency.

The seminal work of Eigen \etal \cite{eigen2014depth} was among the first works introducing modern deep CNNs for the task of monocular depth estimation. The proposed architecture is composed of two stacked networks that predict a depth map from a single RGB image. The first network outputs a coarse depth map and the second network refines its prediction with 3 consecutive convolutions, using the coarse output and the RGB image. Hence, this method is global. Both networks are learned in a fully supervised manner and the final prediction is 4 times smaller than the input. The approach is multi-scale since the output of the coarse network is injected to be refined in the second network.
This work has been extended in \cite{eigen2015predicting} by adding a third scale and combining several tasks, predicting not only depth but also surface normals and semantic labels of the input RGB image. Each task benefits from the others, improving the overall performance.

Several works differ from the ones of Eigen \etal \cite{eigen2014depth} \cite{eigen2015predicting} because their approaches are fundamentally based on local predictions.
Liu \etal \cite{liu2016learning} \cite{liu2015deep} propose a unified deep framework where they train a network to produce both the unary and pairwise potentials of a continuous CRF which regress to depth values. This approach relies on image patches and neighbouring superpixels consistency.
Li \etal \cite{li2015depth} also combine deep CNN with CRF respectively at super-pixel and pixel levels to obtain fine depth maps. They work at the super-pixel level, doing a multi-scale regression with a deep CNN to extract useful features from image patches and estimate a super-pixel depth map. Then, they refine this map to the pixel level using a hierarchical CRF model, enforcing local smoothness.
Roy \etal \cite{roy2016monocular} combine CNN with random forests to do local predictions on the image then fuse the results to obtain the depth map. They input local patches of the image through their random forest and at every tree node they filter the samples with the shallow CNN associated with that node.

On the other hand, some studies have focused on doing both global and local predictions in parallel and then fuse the two estimates to output their final estimation.
Wang \etal \cite{wang2015towards} also addresses the problem of joint depth and semantic prediction to benefit from their complementariness. They refine a global coarse estimation from the whole image and local predictions from regions, the consistency between depth and semantic information being automatically learned through joint training in a two-layer Hierarchical Conditional Random Field (HCRF).
Similarly, Chakrabarti \etal \cite{chakrabarti2016depth} first train a network to output a mid-level representation, characterizing local depth structure by predicting depth derivatives of different orders, orientations and scales from a patch of the original image but also from global scene features. For each derivative, the network produces probability distributions which are then combined using a globalization procedure to estimate the final depth map.

Finally, there have been other global strategies employed like in \cite{eigen2014depth} \cite{eigen2015predicting} to predict the depth map from the whole RGB input image directly in an end-to-end fashion. The state-of-the-art architecture for depth estimation is an encoder-decoder network with a powerful encoder typically trained for semantic purposes. For example, Laina \etal \cite{laina2016deeper} use the ResNet architecture as a feature extractor, cut off the last classification layers and train a decoder on top of it to achieve the regression task of depth prediction. They propose upsampling layers based on the principle of ResNet with skip connections and also show that training with the BerHu loss could improve further the final error. They achieve state-of-the-art on depth estimation from a single monocular image. Although their work achieve impressive results, they do not integrate multi-scale analysis along the network to enhance their prediction.

% \subsection*{Multi-Scale Architectures}
Convolutional architectures that are designed to use multi-scale features all along the network are now well studied in some research areas such as object detection, object recognition and semantic segmentation. We report some of the main contributions that make use of this kind of in-network multi-scale analysis for these tasks.

The U-net \cite{ronneberger2015u} is a popular encoder-decoder architecture where skip connections allow the decoder to benefit from the mirror encoder features (the ones with the same spatial size) to help awareness of finer details. We also study how useful such skip connections can be for the purpose of reconstructing a dense depth map.

Furthermore, Lin \etal \cite{lin2016feature} argue that in addition to skips connections, it is useful to have some intermediate outputs at lower resolution in the decoder, constructing high-level semantic feature maps at different scales. They demonstrate that, at last, it allows to improve both object detection and segmentation tasks. We investigate this approach for the depth estimation task.

On another side, dilated convolutions have been introduced to avoid downsampling in the encoding part of the network while preserving the same receptive field. In some recent work, these benefits were exploited to do a multi-scale analysis by combining features extracted from different scales and with the same spatial size thanks to dilated convolutions \cite{chen2016deeplab}. We use both dilated convolutions to obtain several multi-scale features at the same spatial size along the network and concatenate them to help the decoding stage and also reproduce the spatial pyramid proposed by Chen \etal \cite{chen2017rethinking} to make a comprehensive study on the ideal multi-scale strategy for monocular depth estimation.


==> results.tex <==
\section{Results}
\label{sec:res}

\begin{table}
\begin{center}
\begin{tabular}{|c||c|c|c||c|c|c|}
\hline
\multicolumn{7}{|c|}{\textbf{Classical Metrics Comparison}} \\
\hline\hline
Method & rel & log & rms & $\delta_1$ & $\delta_2$ & $\delta_3$ \\
\hline\hline

%Ours
Single-scale & 0.167 & 0.066 & 0.603 & 77.9 & 94.9 & 98.9 \\\hline
Skips & 0.163 & 0.065 & 0.599 & 79.2 & 95.1 & 98.9 \\
MSML & 0.160 & 0.066 & 0.601 & 78.1 & \textbf{95.4} & \textbf{99.0} \\
FPO & 0.161 & 0.065 & 0.599 & 78.5 & 95.3 & 98.9 \\
DSP & \textbf{0.159} & \textbf{0.064} & \textbf{0.592} & \textbf{79.3} & \textbf{95.4} & 98.9 \\

\hline
\end{tabular}
\end{center}
\caption{Error comparison of the multi-scale methods on the NYU Depth v2 testset. We only use the official subset of 795 training images for the learning stage.}
\label{our_methods}
\end{table}



\begin{table}
\begin{center}
\begin{tabular}{|c||c|c|c||c|c|c|}
\hline
\multicolumn{7}{|c|}{\textbf{Classical Metrics Comparison}} \\
\hline\hline
Method & rel & log & rms & $\delta_1$ & $\delta_2$ & $\delta_3$ \\
\hline\hline

%Eigen \etal 
Eigen \cite{eigen2015predicting} & 0.158 & - & 0.641 & 76.9 & 95.0 & 98.8 \\

%2016
%Liu \etal
%Liu \cite{liu2016learning} & 0.213 & 0.087 & 0.759 & 65.0 & 90.6 & 97.6 \\
%Chakrabarti \etal 
%Chakrabarti \cite{chakrabarti2016depth} & 0.149 & - & 0.620 & 80.6 & 95.8 & 98.7 \\
%Li \etal 
Li \cite{li2017two} & 0.143 & 0.063 & 0.635 & 78.8 & 95.8 & 99.1 \\

%Laina \etal 
%\cite{laina2016deeper} berHu & \textbf{0.127} & \textbf{0.055} & 0.573 \\
%Laina \etal 
Laina \cite{laina2016deeper} \footnotemark & 0.138 & 0.060 & 0.592 & 78.5 & 95.2 & 98.7 \\
%Cao \etal 
Cao \cite{cao2017estimating} & 0.141 & 0.060 & \textbf{0.540} & 81.9 & 96.5 & 99.2\\\hline\hline

%2017
%%Jafari \etal \cite{jafari2017analyzing} & 0.673 \\\hline

Single-scale & - & - & - & - & - & - \\
DSP & \textbf{0.133} & \textbf{0.057} & 0.569 & \textbf{82.3} & \textbf{96.6} & \textbf{99.3} \\


\hline
\end{tabular}
\end{center}
\caption{Comparison of both our single-scale and the best multi-scale methods (DSP) against state-of-the-art results on the NYU Depth v2 testset.}
\label{sota_methods}
\end{table}

\footnotetext{As Laina \etal is the closest method to ours and we train with L2 loss, we only report their results with L2 optimization in this table.}


Here we discuss our results using both the commonly used quantitative metrics, see Table \ref{our_methods} and Table \ref{sota_methods}.

